Robustifying ML-powered Network Classifiers with PANTS

Multiple network management tasks, from resource allocation to intrusion detection, rely on some form of ML-based network traffic classification (MNC). Despite their potential, MNCs are vulnerable to adversarial inputs, which can lead to outages, poor decision-making, and security violations, among other issues. The goal of this paper is to help network operators assess and enhance the robustness of their MNC against adversarial inputs. The most critical step for this is generating inputs that can fool the MNC while being realizable under various threat models. Compared to other ML models, finding adversarial inputs against MNCs is more challenging due to the existence of non-differentiable components e.g., traffic engineering and the need to constrain inputs to preserve semantics and ensure reliability. These factors prevent the direct use of well-established gradient-based methods developed in adversarial ML (AML). To address these challenges, we introduce PANTS, a practical white-box framework that uniquely integrates AML techniques with Satisfiability Modulo Theories (SMT) solvers to generate adversarial inputs for MNCs. We also embed PANTS into an iterative adversarial training process that enhances the robustness of MNCs against adversarial inputs. PANTS is 70% and 2x more likely in median to find adversarial inputs against target MNCs compared to state-of-the-art baselines, namely Amoeba and BAP. PANTS improves the robustness of the target MNCs by 52.7% (even against attackers outside of what is considered during robustification) without sacrificing their accuracy.

==> sections/3-overview-old.tex <==

\section{Overview}
\label{sec:overview}

\maria{add somewhere background on PGD}



\minhao{We not only use PGD but also ZOO. Shall we include bg of both }
Our overarching goal is to \emph{(i)} build an adversarial sample generator which can fulfill all the requirements in \S\ref{sec:requirement}, \emph{(ii)} augment with the generated adversarial samples to robustify the model. 
Since data augmentation has been widely explored and shown strong promise in the networking domain~\cite{jin2022improving}, the main challenge lies in \emph{(i)}. 
Our general idea is to combine canonical AML methods with an SMT solver. \maria{This does not make sense, too early! there is not insight to say that} We first utilize canonical AML methods to generate adversarial features. Given the original sample, the SMT solver is included to find solutions to fulfill those features \maria{weird wording}. These solutions should comply with networking constraints and the threat models. 

\subsection{Why AML + SMT}
\maria{I see that comes from 'Why GANs' but I don't think it makes sense}
The canonical AML methods have been heavily explored in the image domain for several years. \maria{add some background on AML even the actual equation} As shown in table~\ref{tab:requirement}, they have already met most of the requirements. For the networking applications, they can be leveraged to generate adversarial features.
\maria{explain the limitations of only using AML i.e., that there might not be a corresponding packet sequence, even if there exist it might not be realizable given the threat model and even if it is it might not fool the classifier.}
Our question is: \maria{This is not our question! This is our insight} Given those adversarial features, can we formulate the threat model, network constraints and the adversarial features as equations and inequalities for the SMT solver to find solutions. 
So that perturbing the original sample based on the solutions can make its corresponding statistical features adversarial?

SMT seems to be feasible\maria{I don't understand what this sentence says}. It is to determine if the provided mathematical formulas can be satisfiable. Using a SMT solver, we can get a solution or a response\maria{what response?} of no-solution from the formulated equations, \ie if we can perturb the original sample to make its corresponding features equal to or close to the adversarial features. For example, given an original network flow which only has three packets, $f = [p_1^+, p_2^-, p_3^+]$ where $p_i^{\{+,-\}}=(\Delta t_i, l_i)^{\{+,-\}}$, the adversarial features indicate that the average packet length should be $k$. Suppose the threat model only allows to append dummy payload on the forward packets and inject one dummy forward packet at the end of the flow, we thereby define four variables $l_1'$, $l_3'$, $\Delta t^*_4$, $l^*_4$. $l_1'$ and $l_3'$ are representing the appended dummy packet length for $p_1^+$ and $p_3^+$ and $(\Delta t^*_4, l^*_4)^+$ is the new injected dummy packet $p^{*+}_4$. The perturbed flow $f'$ can be formulated as $f'=[\Bar{p}_1^+, p_2^-, \Bar{p}_3^+, p^{*+}_4]=[(\Delta t_1, l_1 + l'_1)^+, (\Delta t_2, l_2)^-, (\Delta t_1, l_3 + l'_3)^+, (\Delta t^*_4, l^*_4)^+]$. Then the formula for the SMT solver is
\begin{empheq}[left=\empheqlbrace]{align}
    & (l_1 + l'_1 + l_2 + l_3 + l'_3 + l^*_4)/4 = k \label{eq:1}\\
    & (l_1 + l'_1 \leq 1500) \wedge (l_3 + l'_3 \leq 1500)  \label{eq:2}\\
    & (40\leq l^*_4 \leq 1500) \wedge (\Delta t^*_4 > 0)  \label{eq:3}\\
    & l'_1 \geq 0 \wedge l'_3 \geq 0\label{eq:4}
\end{empheq}
Equation~\eqref{eq:1} is to fulfill the adversarial features that average packet length after perturbation should be equal to $k$. Equation~\eqref{eq:2} and \eqref{eq:3} align with the network constraint that the maximum packet length should not exceed 1500 bytes and the new injected packet's interarrival times should be larger than 0.
Equation~\eqref{eq:4} complies with the threat model that we can only append payload instead of truncating the existing payload.

After formulation, the SMT solver is expected to return solution(s) or return with "no-solution". The solutions provided by the SMT solver implies a feasible way of perturbation which can fulfill the adversarial features, leading to misclassification. \maria{I think a solution of the SMT provides that there is an reliazable sample. The AML's output is already adversarial!}

\subsection{Challenges and insights}
\label{subsec:insight}
However, naively combing AML and SMT can cause a lot of problems.  Next, we describe the challenges when intergrating AML and SMT into \sys and the corresponding insights.

\begin{challenge}
    The canonical AML methods cannot capture the cross dependencies between the features and also cannot understand the networking constraints and threat models.
\end{challenge}

The feature engineering module extracts multiple features to describe the statistical pattern of the network sample. Table~\ref{tab:dataset} shows several examples of the extracted features in different applications. Usually, these features have strong statistical dependency, \eg $max \geq mean \geq min$ of interarrival times. Breaking these interdependency\maria{what do you mean break the dependency WHY?} can directly lead to a failure of getting any solution when using the SMT solver. For example, if the adversarial features given by AML methods show that $mean > max$ of interarrival times, there is no way to find a solution to both fulfill these two features. Moreover, the adversarial features fed into the SMT solver should also comply with the networking constraints and the threat model. For example, suppose \{number of bytes per second, number of packets per second\} are two of the extracted features, average packet length can be derived by number of bytes per second / number of packets per second, which cannot be less than 28 for a UDP flow and 40 for a TCP flow. Also, if \{duration, number of packets per second\} are extracted, the number of packets can be derived by duration / number of packets per second. It cannot be smaller than the number of packets in the original flow since the threat model doesn't allow dropping packets.
Violating any networking constraints and the threat model can also lead to a failure on getting any solutions.

Unfortunately, AML fails to capture the dependencies between features and cannot force the generated features to comply with the constraints and threat model because they cast each feature independently. \maria{you start this section by saying naivily combining SMT with AML is not good enough. Not only AML is not good enough!} Adding Lagrangian terms into the target loss function is a potential way to improve that, \ie $loss = loss + \alpha * (max - mean)$ where $\alpha > 0$. Since AML is targeting at increasing the loss, it should try its best to increase the max and decrease the mean of interarrival times. However, we argue that this method has very limited effect on maintaining the dependency. First, adding Lagrangian terms cannot fully avoid the situation that $mean > max$ but only mitigate it. Second, it's not trivial to satisfy a full spectrum of dependencies, networking constraints and the threat model, since some of them are convoluted and hard to formulate. For example, what can be the correlation of interarrival times for the bi-directional flow and its forward and backward subflow given that the attacker can only delay the forward packets? 

\begin{insight}
    Selecting a subset of adversarial features are feasible for a SMT solver to return solutions without sacrificing adversariness.
    \label{insight:1}
\end{insight}

Since the adversarial features generated by AML can easily violate dependencies, networking constraints and the threat model, using the whole set of features for solutions is likely to fail. An alternative way is to consider using a subset of features. The selection of features to form a subset should meet two requirements. (1) Fulfilling the features in the subset are enough to be adversarial (2) These features should comply with the dependency, constraints and threat model, \ie the SMT solver can return solutions.  Hence, we design an algorithm to choose important features on maintaining adversariness and then check if these selected features are viable for the SMT solver to return solutions. It generally includes two parts, feature importance ranking and adaptive SMT verification. 

\myitem{Feature importance ranking} Given adversarial features, different features may not be equally important on keeping the flow adversarial. For example, suppose there is a VPN flow $f$ and its extracted features are mean and max of interarrival times, \ie [$mean_{iat}$, $max_{iat}$]. The AML method changes these two features to be $mean'_{iat}$ and $max'_{iat}$ so that it is classified as Non-VPN. Unfortunately, the SMT solver returns no-solution when fulfilling these two features. Instead of directly returning to users that \sys cannot find adversarial samples, we want to try if the SMT solver can return a solution on fulfilling one of the features. And another feature can be calculated by feature engineering the adversarial flow generated from the solution. For example, suppose $mean'_{iat}$ is more important than $max'_{iat}$, then we ask the SMT solver to provide solutions on fulfilling $mean'_{iat}$. After that, we construct the adversarial flow using the solution and then apply feature engineering on it to recalculate another feature $max''_{iat}$. Since the most important feature on keeping adversariness, $mean'_{iat}$, is kept, we hope that the new adversarial feature [$mean'_{iat}$, $max''_{iat}$] can still be adversarial. Therefore, we design an algorithm to determine what features are important and ask the SMT solver to provide solutions only on the important features.  Since AML methods are designed to perturb features to increase loss following the direction of the (approximated) gradient and the gradient is known to be the steepest direction on changing the loss, our intuition is that the features which have been changed a lot plays an important role for adversariness.  Therefore, we design a feature importance ranking algorithm based on the extent of change for each feature between the original and adversarial one. After normalizing all the features into the same scale, the importance for each feature is determined by the difference of that feature value between the adversarial and the original one. 

\myitem{Adaptive SMT verification} \maria{what is verification here?!} After we rank the importance of each feature, we still cannot answer a critical question. Once we select some important features, how to make sure the selected features are possible to have solutions? Therefore, we design an adaptive SMT verification algorithm. This algorithm is running in an iterative way. We first construct a list to represent the selected features and it is empty at the beginning. Each time, the list will be appended with the $i$th most important feature $f_i$ and check if SMT can provide solutions on fulfilling the features in the updated list. If not, the list removes $f_i$.
% since SMT can find solutions on all the remaining features in this list and all of them are more important then it. 
This procedure will continue until the first $k$ important features are tried. $k$ is a parameter set by the users, basically it can be any number between 1 and number of features. However, setting it as a small value forces the algorithm include only very few features which can hurt the adversariness. Setting it too large includes too many non-important features, making the generation speed slow without much adversariness improvement. 

Our intuition is that we always want to include important features into the selected features list to keep the the solution returned by the SMT adversarial. But if the SMT solver cannot return solution after the new feature is added,it may due to the conflict of statistical interdependency, constraints or the threat model. Then we can only pop it out from the list. 
The pseudocode of the algorithm is described in alg~\ref{alg:feat_selection}. It's possible that after appending $f_i$, the solution provided by the SMT solver is already adversarial. However, in order to cover a wider spectrum of adversarial features, the algorithm collects this solution and continue appending $f_{i+1}$ for another potential solution until $i$ reaches $k$.

Figure~\ref{fig:insight1-loss} shows the CDF of loss under different threat models (strong and weak attacker's capabilities) in three diverse applications.  The loss is defined as the Cross Entropy between the adversarial samples' predicted probabilities of labels and the ground truth labels. A higher loss indicates larger possibility to be adversarial. We compare the results with the baseline Amoeba. The training mechanism of the agent from Amoeba also includes maximizing the cross entropy (defined in reward function). So it's useful to compare with Amoeba to evaluate \sys's ability on generating samples with high loss. Since Amoeba can only generate one adversarial sample for each benign one, for a fair comparison, we include the original sample's loss (which is very small) if \sys cannot generate one single adversarial sample from it and pick the one with the largest loss if \sys generates multiple ones. Compared to Amoeba, \sys is able to generate high-loss adversarial samples with larger support in the Application Identification (APP) and VPN detection (VPN). \sys also perform betters than Amoeba under weak capability for VCAs QoE Inference (QOE) and achieves similar performance with Amoeba under strong capability. 


\begin{algorithm}
\caption{Adaptive SMT verification}\label{alg:feat_selection}
\scriptsize
\begin{algorithmic}
\State SMT\_solver $\gets$ a SMT solver returning solutions or null on fulfilling the selected features.
\State k $\gets$ Maximum number of important features considered
\State sorted\_feature\_list $\gets$  ($f_1$, $f_2$, ..., $f_n$)
\Comment{Sorted by importance descending order}
\State selected\_features $\gets$ ()
\For{$i$ in 1:k} \Comment{$k \leq n$}
    \State selected\_features.append($f_i$)
    \If{SMT\_solver(selected features) is null}
        \State selected\_features.remove($f_i$)
    \Else 
        \State Collect the solution
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{figure}[htp]
\centering
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/insight1-app.pdf}  
    \caption{APP}
    \label{}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/insight1-vpn.pdf}  
    \caption{VPN}
    \label{}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/insight1-vca.pdf}  
    \caption{QOE}
    \label{}
\end{subfigure}
\caption{The CDF of the generated samples' loss by \sys and Amoeba under different attackers' capabilities and applications. Selecting a subset of the most important features can generate adversarial samples with high loss. \sys has  higher support than Amoeba on generating high-loss adversarial samples. }
\label{fig:insight1-loss}
\end{figure}

\begin{challenge}
    The generation speed is hindered by the SMT solver, which slows down when processing complex formulas.
\end{challenge}

The speed of generating adversarial samples is an important factor for \sys to be usable. However, SMT is not always able to find a solution or return with no-solution in a short period. In some cases, SMT is running for a long time to return or even hangs. This may due to high calculation complexity based on the given formula. The complexity depends on many factors such as the length of the network flow, the number of features needs to be solved and the difficulty of solving each feature. First, a longer network flow requires more variables to represent the permissble actions for each packet, which implies a much larger search space for the SMT solver to return solutions. This generally requires more time for the SMT to compute. Second, including more features into the feature set for solutions means that more equations and inequalities need to be satisfied. This potentially increase the time for SMT to compute. Third, solving each feature is not equally difficult for the SMT solver. For example, solving the basic statistics (\ie max, min, mean, median) of packet length is easier than calculating the number of unique packet length. Moreover, situations can be even worse when these factors are overlapped.

However, naively applying timeout mechanism to set a hard time budget can control the generation time under a reasonable duration, but it has negative influence on adversariness since any computation which takes longer than the timeout budget returns without an adversarial sample.

Moreover, some capabilities defined by the threat model may require the SMT to run multiple times, which worsen the generation speed. For example, when the treat model allows the attacker to inject at most 20 packets at the end of the flow, the SMT solver is expected to run 21 times (iterating from injecting 0 packet to 20 packets) to get most of the possible solutions in order to cover a full spectrum of adversarial features. Sequentially running multiple times makes the adversarial sample generation speed even slower.

\begin{insight}
    Generation speed can be optimized by the combination of timeout mechanism, network flow chunking and parallel computing. \label{insight:2}
\end{insight}

Since the SMT solver is the main bottleneck of the generation speed, effort is spent to optimize this part. Although timeout mechanism is suboptimal for adversariness, it is a good indicator to reflect the computation complexity. Once we find that SMT cannot return anything within a timeout window, we try to decrease the computation complexity by splitting a flow into several chunks evenly. The SMT solver is leveraged to provide solutions for each chunk. Since each chunk has fewer packets compared to the whole flow, it's more likely that the SMT solver is able to return solutions in a short time. However, chunking also has tradeoffs. After splitting a flow into multiple ones, some features are difficult to be formulated strictly. For example, when solving on a complete flow, it's easy to fulfill the feature, maximum of packet length. After splitting the flow into multiple chunks, the maximum of packet length can be one packet appearing in any chunks. Strictly solving this problem would require a complicated algorithm, which is in conflict with our motivation for chunking. To solve this problem, we just try a naive way. We first split features into three different types. 
The first type belongs to the features that fulfilling them in each chunk can make the whole flow roughly have the same values. For example, \{max, mean, median, min, std\} of \{interarrival times, packet length\} and number of \{packets, bytes\} per second can all be considered as this type of features. For these features, SMT solves on them per chunk. 
The second type is features that summing them up for each chunk is equal to that for the whole flow. One typical example is the duration. For these features, we just ask each chunk to fulfill $\frac{feature}{\#chunks}$ since chunks are splitted evenly. 
Other features doesn't belong to the first two types such as number of unique packet length will be ignored by the SMT solver when it is leveraged to solve on each chunk instead of the whole network flow.

Finally, the generation time can be further sped up by using parallel computing. Since the SMT solving process for each flow/chunk is designed to be independent, parallel computing can be fully utilized. Figure~\ref{insight:2} shows the generation speed after optimization. \sys achieves reasonable efficiency by taking less than 0.6s on generating a single adversarial sample in most of the cases.


\begin{figure}[htp]
\centering
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/efficiency_APP.pdf}  
    \caption{APP}
    \label{}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/efficiency_VPN.pdf}  
    \caption{VPN}
    \label{}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/efficiency_QOE.pdf}  
    \caption{QOE}
    \label{}
\end{subfigure}
\caption{The average generation time per adversarial sample is less than 0.6s for almost all the ML models in the three selected applications. The SVM model in the application QOE is the only exception. The generation speed doesn't have notable difference between capabilities.}
\label{fig:insight2-speed}
\end{figure}

\begin{challenge}
    Some attacker's capabilities are inefficient to compute.
    \label{challenge:3}
\end{challenge}

Unfortunately, not all the capabilities can be formulated and efficiently computed by the SMT solver. The capability to inject packets at any position is one of them. The underlying reason is that multiple dummy packets can be injected at any position, covering a full combination of all the positions requires huge amount of computation. For example, suppose a network flow has $k$ packets and $m$ dummy packets are expected to be injected, except injecting at the front of the flow, there are k positions available for the dummy packets to inject. This is a typical "stars and bars" problem~\cite{startsbars} and the total number of different combination are $\binom{m+k}{m}$. With a fixed $m$, the time complexity on covering all the combinations is $O(k!)$, indicating large number of combinations and heavy computation when the flow is long. This is even worse when the threat model allows to inject at most j packets, then the total number of combination is $\sum_{k=0}^{j}\binom{m+k}{m}$. Thereby, packets injection at any position is very inefficient. A strict implementation affects usability.

\begin{insight}
    The second advantage of leveraging chunking: Inefficient and complicated capabilities applied on the whole flow can be approximately implemented as simple capabilities applied on each chunk.
\end{insight}

As explained in \challengeref{challenge:3}, packets injection at any position is inefficient. However, there is one exception, which is injecting packets at the end of the flow. Since there is only one position possible for injection, the SMT solver only needs to compute once to return the solutions.
Therefore, we borrow the idea of chunking in \insightref{insight:2}. 
We approximated implement the packets injection at any position as packets injection at the end of each chunk. As we decrease the number of packets per chunk, the number of chunks increase and the final effect is closer to packets injection at any place.

==> sections/7-related.tex <==
\vspace{-0.25cm}
\section{Related work}
\label{sec:related}
\vspace{-0.3cm}

%Owing to their stability and usability, 
AML methods, including 
FGSM~\cite{goodfellow2014fgsm}, PGD~\cite{madry2017pgd}, and ZOO~\cite{chen2017zoo}, are effective against ML models operating in the image domain. Such approaches create perturbations for each sample to maximize the loss of the target model. Unfortunately, directly using these techniques to target ML models of networking applications would often result in infeasible adversarial examples in practice, as discussed in \S\ref{subsec:limit_existing_work},\S\ref{subsec:aml-promise}. %is questioning on its correctness and faithfulness\maria{what is questioning?}. 
%Indeed, multiple networking applications include a complicated, non-invertible feature-engineering module that precedes the ML model. As a result, features cannot be changed independently from each other, nor can they have arbitrary values, as they describe real traffic, and are thus interdependent and constrained by multiple domain rules. 
%For instance, one cannot change median and average interarrival times independently. 
%The features fed into the ML model have strong constraints, such as dependencies between features and domain-specific rules. 
%In essence, methods such as  consider each feature independently, which can easily violate the constraints. Moreover, there is no guarantee that the perturbed features can correspond to its original flow under the perturbation within a realistic threat model. 



Inspired by FGSM and GAN, Blind Adversarial Perturbation (BAP)~\cite{BAP} trains a perturbation generator, which can generate practical attacks against end-to-end Deep Neural Network-based website fingerprinting and flow correlation calculation. 
Unlike the methods previously mentioned, BAP is able to perturb flows at the packet level and incorporate networking constraints. BAP trains a perturbation generator to produce adversarial flows. It designs regularizers and remapping functions to adjust the perturbed network to enforce networking constraints. However, the targeted ML model needs to directly accept packet timings, packet size and directions as input. Any application that has non-differentiable and non-invertible parts, such as a feature engineering module or not using Neural-Network-related ML, is not applicable to this method. 

Amoeba~\cite{amoeba} is an RL-based attacker against ML-powered censorship. The agent perturbs each packet to maximize the chance that a flow is misclassified. While it can generate samples that deceive models that include feature engineering, those samples cannot be used for improving the robustness of the model. Moreover, similar to other RL-based methods, Amoeba suffers from instability in training, making it less usable. Finally, Amoeba results are hard to interpret, as it is hard to explain why specific actions lead to adversarial examples.


Training a robust model against adversarial attacks is an important topic being explored heavily in the image domain. %Multiple different strategies have been proposed, such as adversarial training and robustness certification.
%
%\mypara{Adversarial training} 
Adversarial training~\cite{madry2017pgd,jeddi2020simple,wong2020fast,li2023data,shafahi2019adv4free} is the process of generating adversarial samples corresponding to the original dataset and then augmenting the original training set with the adversarial counterparts to build a more robust model. 
%Although we are the first to propose a specialized framework for networking applications, there are efforts as a method of attack on generating adversarial samples.
%
%\mypara{Robustness certification}
Robustness certification works~\cite{li2023sokcertified,wang2021betacertified,xu2020automaticcertified,tjeng2017evaluatingcertified,yang2020randomizedcertified} have a theoretical proof that the ML model will remain stable and reliable within a robustness region against perturbation. BARS~\cite{wang2023bars} is one of the frameworks that provide a robustness guarantee for \NetApps, which have feature engineering. However, it only considers the robustness guarantee at the feature level instead of the guarantee at the packet level. Therefore, a small perturbation in the flow, such as injecting a dummy packet in a small interarrival time, can easily exceed its robustness region in the feature space. Also, certified robustness cannot match the empirical robustness using adversarial training~\cite{wong2020fast, nandy2021towards}


%The robustification process of ML models, known as adversarial training, similar to this work, relies on the generated adversarial samples. Several different ways of using the adversarial samples have been proposed in the image domain to robustify the models. For example, NN-based models are usually robustified by substituting the original sample with its adversarial counterpart during each training iteration to update the model parameters~\cite{madry2017pgd}. Other ways, such as fine-tuning the trained model with adversarial samples or augmenting the original dataset with their adversarial counterparts to retrain a more robust model, are also popular~\cite{jeddi2020simple,li2023data,zhao2020maximum}.
